Complexity of Supersymmetric Systems and the Cohomology Problem

We consider the complexity of the local Hamiltonian problem in the context of fermionic Hamiltonians with $\mathcal N=2 $ supersymmetry and show that the problem remains $\mathsf{QMA}$-complete. Our main motivation for studying this is the well-known fact that the ground state energy of a supersymmetric system is exactly zero if and only if a certain cohomology group is nontrivial. This opens the door to bringing the tools of Hamiltonian complexity to study the computational complexity of a large number of algorithmic problems that arise in homological algebra, including problems in algebraic topology, algebraic geometry, and group theory. We take the first steps in this direction by introducing the $k$-local Cohomology problem and showing that it is $\mathsf{QMA}_1$-hard and, for a large class of instances, is contained in $\mathsf{QMA}$. We then consider the complexity of estimating normalized Betti numbers and show that this problem is hard for the quantum complexity class $\mathsf{DQC}1$, and for a large class of instances is contained in $\mathsf{BQP}$. In light of these results, we argue that it is natural to frame many of these homological problems in terms of finding ground states of supersymmetric fermionic systems. As an illustration of this perspective we discuss in some detail the model of Fendley, Schoutens, and de Boer consisting of hard-core fermions on a graph, whose ground state structure encodes $l$-dimensional holes in the independence complex of the graph. This offers a new perspective on existing quantum algorithms for topological data analysis and suggests new ones.

==> qm.tex <==
% !TEX root = ./SUSY_Complexity.tex

%%%%%%%%%%%%%%%%%%%%
\section{Supersymmetric Quantum Mechanics}
\label{sec:Supersymmetric Quantum Mechanics}

We begin by reviewing basic aspects of supersymmetric quantum mechanics  \cite{Nicolai:1976xp, Witten:1981nf,Witten:1982df,Witten:1982im}, including the supersymmetric algebra,  the structure of ground states and  the role of cohomology. We mostly follow the original exposition in \cite{Witten:1982df,Witten:1982im} and also Chapter 10 of  \cite{Hori:2003ic}.\footnote{See also \cite{JunkerSUSYBook} for a textbook focusing on applications of supersymmetry to statistical mechanics.}
 


\subsection{Definition, algebra, and spectrum}

The Hilbert space of  any quantum mechanical theory can be decomposed as 
\equ{\label{HFB}
\cH= \cH^{B}\oplus \cH^{F}\,,
}
where $\cH^{B}$ and $\cH^{F}$ are the spaces of bosonic and fermionic states, respectively. These are distinguished by an operator, denoted $(-1)^{F}$, which  acts  as $+1$ on bosonic states and as $-1$ on fermionic states.  By definition, a supersymmetric quantum mechanics is a quantum mechanical system in which there is a set of Hermitian operators, $Q_I$, $I=1,\ldots,\cN$, sending states in $\cH^{B}$ into states in $\cH^{F}$ and vice versa. The operators $Q_{I}$ are the generators of supersymmetry, or ``supercharges,'' and one says that the quantum mechanics has $\cN$ real supercharges.  A basic consistency requirement is that 
\equ{\label{QF}
\{(-1)^{F},Q_I\}=0\,,
}
where $\{\cdot,\cdot\}$ is the anticommutator. In addition, one imposes that the supercharges satisfy the algebra
\equ{\label{qiqjH}
\{Q_I,Q_J\} =\delta_{IJ}\, H\,,\qquad I,J\in\{1,\ldots,\cN\}\,,
}
where $H$ is, by definition,  the Hamiltonian of the system. In words, an $\cN=1$ supersymmetric Hamiltonian is thus a Hamiltonian that can be written as the {\it square} of a parity-odd operator $Q$. If there are $\cN$ such independent operators, all anticommuting with each other,  then one says that the systems ``has $\cN$ real supercharges.'' 

It follows directly from the algebra above that
\equ{
[Q_{I},H]=0\,,\qquad [(-1)^{F},H]=0\,,
}
and thus the operators $Q_{I}$ and $(-1)^{F}$ are symmetries of such systems. Another crucial property of supersymmetric systems is that the spectrum is positive semi-definite:
%\equ{
%\bra{\psi}H\ket{\psi}=\frac{1}{\cN}\bra{\psi}\sum_{I=1}^{\cN}\{Q_{I},Q_{I}\}\ket{\psi}=\frac{2}{\cN}\sum_{I=1}^{\cN}\norm{Q_{I}\ket{\psi}}^{2}\geq 0\,.
%}
\equ{
\bra{\psi}H\ket{\psi}=\bra{\psi}\{Q_{I},Q_{I}\}\ket{\psi}=2\norm{Q_{I}\ket{\psi}}^{2}\geq 0\,,\qquad \text{for each $I$.}
}
In particular, a state $\ket{\Omega}$ has $E=0$ if and only if it preserves all the supersymmetries, i.e., 
\equ{\label{qomega0}
Q_{I}\ket{\Omega}=0\,, \qquad \qquad \qquad I=1,\ldots,\cN\,.
}
Such states, if they exist, are called {\it supersymmetric ground states}. 



\begin{figure}
\begin{center}
\includegraphics[scale=1.6]{Figures/spectrum.pdf}
\put(-85,130){bosonic} \put(-30,130){fermionic}
\put(-130,50){$E>0$}
\put(-130,0){$E=0$}
\caption{The spectrum of supersymmetric quantum mechanics. Black dots represent bosonic states and white ones fermionic states. All states with $E>0$ come in boson/fermion pairs.  Supersymmetric ground states ($E=0$), if there are any, are not necessarily paired.}
\label{fig:spectrum}
\end{center}
\end{figure}

A crucial property of  states with $E>0$ is that they come in boson-fermion pairs with the same energy. To see why this is the case consider for example a bosonic state $\ket{b}$ with $E>0$ and thus there exists at least one supercharge, say  $Q\equiv Q_{1}$, which does not annihilate the state. Then, the fermionic state  $\ket{f}\equiv \frac{1}{\sqrt E}Q\ket{b}$ is normalized and has the same energy as $\ket{b}$, since $Q$ commutes with the Hamiltonian. One then says that the states  $(\ket{b},\ket{f})$ form a ``supersymmetric doublet'' and furnish a two-dimensional representation of supersymmetry. When there are several supercharges one may apply multiple $Q_{I}$'s, obtaining a longer multiplet of bosonic and fermionic states but these can be constructed by combining  doublets for each supercharge. The conclusion is that, regardless of the total number of supercharges, for each bosonic state with $E>0$ there is a corresponding fermionic state with the same energy (see Figure~\ref{fig:spectrum}).\footnote{In this paper we shall be mostly interested in finite-dimensional Hilbert spaces and thus the spectrum is discrete.}


The situation for supersymmetric ground states, $E=0$, on the other hand,  is very different. As seen above,  in this case the supercharge annihilates the state, $Q\ket{\Omega}=0$, and thus  supersymmetric ground states cannot be paired into  doublets. Rather,  they  stand by themselves, in the trivial representation of supersymmetry. Thus, in general there can be an arbitrary number, $n_{E=0}^{B}$ and $n_{E=0}^{F}$, of bosonic and fermionic supersymmetric ground states, respectively. An important quantity is the Witten index, defined as the difference in the number of bosonic and fermionic supersymmetric ground states \cite{Witten:1982df},
\equ{
\cI \equiv n^{B}_{E=0}-n^{F}_{E=0}\,. 
}
The quantum mechanical system  of  Figure~\ref{fig:spectrum}, for instance, has Witten index $\cI=4-2=2$. Computing the Witten index, given a local supercharge and an efficient description of the Hilbert space as input, is $\#\P$-complete  \cite{Crichigno:2020vue}.

\

It is useful to distinguish operators acting on the Hilbert space according to the action of $(-1)^{F}$ on the operator. An operator  is said to be bosonic or fermionic if it commutes or anticommutes with the parity operator, i.e.,  
\equ{
[(-1)^{F},\cO_{B}]=0\,,\qquad \qquad \{(-1)^{F},\cO_{F}\}=0\,,
}
respectively. It follows that when acting on a state with definite parity, bosonic operators preserve its parity and fermionic operators flip it. The supercharges $Q_{I}$, for example, are fermionic operators and the Hamiltonian is a bosonic operator.

%\paragraph{The Witten index.}  The Witten index  \cite{Witten:1982df} is defined as the {\it difference} in the number of bosonic and fermionic  ground states,
%\equ{\label{defWitten}
%\cI\equiv  n_{E=0}^B-n_{E=0}^F=\text{Tr}_{\cH}\, (-1)^F \,.
%}
%In the second equality  the Witten index has been written as sum over {\it all} states in the theory, including those with $E>0$. This is because, as noted above,  these come in boson-fermion pairs and  their contributions in the trace thus cancel out.\footnote{More precisely, for systems with an infinite spectrum one inserts a regulating factor $e^{-\beta H}$ to ensure convergence of the sum. Written in this form, the Witten index can be interpreted as the  partition function of the theory, where the purpose of  $(-1)^{F}$ is to impose periodic boundary conditions on fermionic states (rather than the more standard antiperiodic ones), to match that of bosonic states and preserve supersymmetry. The index is independent of $\beta$ and so one can take the limit $\beta\to 0$ at the end of the calculation (see \cite{Witten:1982df} for more details). We will focus here on systems with a finite spectrum where the issue of convergence does not arise and we set $\beta=0$. } An important consequence of this is that the Witten index can thus be evaluated without knowledge of the supersymmetric ground states; one simply takes the alternating sum over {\it all} states in the Hilbert space and supersymmetry ensures this matches the difference in the number of bosonic and fermionic ground states. 
%
%\
%
%The sign of the Witten index indicates an excess of either bosonic or fermionic ground states and its magnitude gives a lower bound on the total number of ground states, via the inequality
%\equ{\label{WittenboundGS}
%n_{E=0}^{B}+n_{E=0}^{F}\geq \abs{\cI}\,.
%}
%In particular, if $\cI\neq 0$ one learns that the system {\it must} have supersymmetric ground states. If $\cI=0$  the bound is trivial; one simply learns that $n_{E=0}^{B}=n_{E=0}^{F}$, but this number may be zero. 
%
%
%\
%
%
%A crucial  property of the Witten index is that it is a robust quantity under continuous deformations of the system, as long as the deformation preserves supersymmetry.\footnote{There are important exceptions to this property but it is often valid under reasonable assumptions. See the discussion in  \cite{Witten:1982df}.   }  For instance, if a ground state is to become an excited level, it can only do so if it can ``pair up'' with another  state of opposite statistics, and  same energy, so that excited levels continue to be paired, as required by supersymmetry. The number of bosonic and fermionic ground states are then both decreased by 1 but the Witten index is unchanged.  Similarly, if an excited state is to  become a ground state it can only do so  provided its partner moves too, so that no unpaired states are left behind, and the Witten index is again  unchanged by this process.  Such robustness is typical of supersymmetric systems. It is this property that makes computing the Witten index often feasible, especially for systems admitting a supersymmetric deformation  to a weakly coupled point where computing the index is straightforward. Nevertheless, as we discuss below,  the Witten index problem is in general computationally hard.
%



\paragraph{$\cN=2$ systems. } From now on we will focus on systems with $\cN=2$ supersymmetry. In this case it is useful to combine the Hermitian supercharges into the complex combinations 
\equ{
\cQ\equiv \frac{1}{\sqrt 2} (Q_1+ i Q_2)\,,\qquad \cQ^\dagger\equiv\frac{1}{\sqrt 2} (Q_1- i Q_2)\,.
}
The supersymmetry algebra \eqref{qiqjH} implies these complex supercharges are nilpotent of degree two, i.e., 
\equ{\label{nilpQ}
\cQ^{2}=(\cQ^{\dagger})^{2}=0\,.
}
The Hamiltonian can be written as
\equ{\label{QQcom}
H=\{\cQ,\cQ^\dagger\}\,.
}
%The supercharges $\cQ$ and $\cQ^{\dagger}$ have fermion number $+1$ and $-1$, respectively,
%\equ{
%[F,\cQ]= \cQ\,,\qquad [F,\cQ^{\dagger}]= -\cQ^{\dagger}\,,
%}
%and therefore the Hamiltonian preserves the fermion number,  $[F,H]=0$.
%
%\
As discussed above, supersymmetric ground states (states with exactly zero energy) must preserve all supersymmetries and thus
\equ{\label{SUSYgs}
\cQ\ket{\Omega}=\cQ^\dagger\ket{\Omega}=0\,.
} 
One of the most important properties of $\cN=2$ supersymmetric quantum mechanics is that supersymmetric ground states are in one-to-one correspondence with the cohomology group of $\cQ$. We review this next.  


\subsection{Supersymmetric ground states and cohomology}
\label{sec:Cohomology, homology, and ground states}

%Many of the  robustness properties of supersymmetric systems are due to certain observables being topological in nature and thus invariant under continuous deformations. The  Witten index is such an example. Indeed, the  problem of characterizing the space of supersymmetric ground states, $\cH_{E=0}$, can be formulated as  that of computing the  cohomology group of $\cQ$ (or, equivalently, the homology group of $\cQ^{\dagger}$) and the Witten index equals the Euler characteristic of the corresponding cochain complex. Let us briefly review this relation.\footnote{Here we mostly follow  Chapter 10 in the book  \cite{Hori:2003ic}. .}

Consider the set of states in the kernel and image of $\cQ$, i.e., 
\equ{
\text{Ker}(\cQ)= \{\ket{\psi}\;|\; \cQ\ket{\psi}=0\}\,,\qquad \text{Im}(\cQ)= \{\ket{\psi}\;|\; \ket{\psi}=\cQ\ket{\psi'}\}\,,
}
where $\ket{\psi'}$ is some state. States in $\text{Ker}(\cQ)$ are said to be ``$\cQ$-closed'' and states in $\text{Im}(\cQ)$ are said to be ``$\cQ$-exact.'' (The same definitions hold  for  $\cQ^{\dagger}$ and supersymmetric ground states \eqref{SUSYgs} are closed with respect to both $\cQ$ and $\cQ^{\dagger}$.) Now, since $\cQ^{2}=0$, all states that are $\cQ$-exact are also $\cQ$-closed and thus $\text{Im}(\cQ)\subseteq\text{Ker}(\cQ)$. Then, the  vector space 
\equ{
H(\cQ)\equiv \frac{\text{Im}(\cQ)}{\text{Ker}(\cQ)}
} 
is well defined and known as the {\it cohomology group} of $\cQ$.\footnote{In this case the cohomology group has the additional structure of a vector space but this is not necessary. See Section~\ref{The k-local cohomology problem} for the general definition. }  It consists of all states in the Hilbert space which are $\cQ$-closed but not $\cQ$-exact. 
% in the two important notions are those of closedness and exactness. One defines:
%\eqss{\label{QStates}
%\text{$\cQ$-closed:}\quad \cQ\ket{\psi}=0\,,\qquad\qquad\qquad
%\text{$\cQ$-exact:} \quad \ket{\psi}=\cQ\ket{\psi'}\,,
%}
%where $\ket{\psi'}$ is some state. 
%
% It is straightforward to see that all exact states are closed. The converse, however,  is not necessarily true. and cannot be exact. 
In fact, due to the $\Bbb Z_{2}$-grading of the Hilbert space, $\cH=\cH_{B}\oplus \cH_{F}$, there is a more refined structure and one can define $\Bbb Z_{2}$-graded ``complex''  of vector spaces,
\equ{\label{complexBF}
C: \qquad \cH^{F}\xrightarrow{\cQ}\cH^{B}\xrightarrow{\cQ}\cH^{F}\xrightarrow{\cQ}\cH^{B}\,.
}
Then, one can define two cohomology groups:
\eqs{
H^{B}(\cQ)\equiv\,& \frac{\text{Ker}(\cQ): \cH^{B}\to \cH^{F}}{\text{Im}(\cQ): \cH^{F}\to \cH^{B}}\,,\\ 
H^{F}(\cQ)\equiv\,& \frac{\text{Ker}(\cQ): \cH^{F}\to \cH^{B}}{\text{Im}(\cQ): \cH^{B}\to \cH^{F}}\,,
}
consisting of all bosonic and fermionic states which are $\cQ$-closed but not $\cQ$-exact, respectively. The full cohomology group is 
\equ{
H(\cQ)=H^{B}(\cQ)\oplus H^{F}(\cQ)\,.
} 
A  complex for which $\text{Ker}(\cQ)=\Im(\cQ)$, and thus $H(\cQ)=0$,  is called an {\it exact} sequence. Thus, cohomology groups are a measure of the failure of a  sequence to be exact.\footnote{For a textbook on algebraic topology see, e.g., \url{http://pi.math.cornell.edu/~hatcher/AT/ATplain.pdf} and for computational aspects see \cite{CompTopBook,zomorodian_2005}.}
%pedagogical introduction to homology and cohomology see, e.g., \url{https://www.seas.upenn.edu/~jean/sheaves-cohomology.pdf}, .}  



Physically, an exact sequence corresponds to a system with no supersymmetric ground states. To see this, note that states with $E>0$ that are $\cQ$-closed  are necessarily $\cQ$-exact, as follows directly from the supersymmetry algebra \eqref{QQcom}. Indeed, applying the algebra  on a state with energy $E$ one has $\{\cQ,\cQ^\dagger\}\ket{\psi}=E\ket{\psi}$. Using that the state is $\cQ$-exact and assuming $E>0$, implies $\ket{\psi}= \cQ \ket{\psi'}$ with $\ket{\psi'}\equiv \frac{1}{E} \cQ^\dagger \ket{\psi}$ and thus the state $\ket{\psi}$ is  $\cQ$-exact.  On the other hand, all  states with $E=0$ are necessarily closed, as we have already seen, but   {\it cannot} be exact. To show this  suppose for the sake of contradiction that is the case, i.e., that there exists a state $\ket{\psi'}$ such that $\ket{\Omega}=\cQ\ket{\psi'}$. Since $\cQ$ commutes with $H$, the state $\ket{\psi'}$ must also have $E=0$ and hence must be $\cQ$-closed,  $\cQ\ket{\psi'}=0$. The upshot of this analysis is that $\text{Ker}(\cQ)|_{E>0}=\text{Im}(\cQ)|_{E>0}$ while  $\text{Im}(\cQ)|_{E=0}=0$. These two statements together imply
\equ{
 H^B(\cQ)= \cH^B_{E=0}\,,\qquad \qquad  H^F(\cQ)= \cH^F_{E=0}\,,
}
as claimed.  That is, the cohomology of  $\cQ$ is given by the set of supersymmetric ground states. In particular, the total number of SUSY ground states is given by the dimension of the full cohomology group,
\equ{
n_{E=0}^{B}+n_{E=0}^{F}=\dim H^{B}(\cQ) +\dim H^F(\cQ)\,,
}
while the Witten index of the system can be written as 
\equ{\label{Wcoh}
\cI= n_{E=0}^{B}-n_{E=0}^{F}= \dim H^B(\cQ)- \dim H^F(\cQ)\,,
}
which is known as the {\it Euler characteristic} of the complex \eqref{complexBF}. To summarize, finding the space of supersymmetric ground states is equivalent to finding the cohomology group $H(\cQ)=H^{B}(\cQ)\otimes H^{F}(\cQ)$ and computing the Witten index is equivalent to computing the Euler characteristic of the associated complex. 



\paragraph{Systems with $F\in \Bbb N_{0}$.} In certain models, a more refined structure may appear. A case of particular interest to us is when there exists an operator $F$   (usually called the fermion number operator)  with integer-valued eigenvalues, $\Bbb N_{0}=\{0,1,\cdots\}$, and thus one can identify the parity operator $(-1)^{F}$, literally as ``minus one to the power $F$, '' or
\equ{
(-1)^{F}=e^{i\pi F}\,.
}
The Hilbert space can then be graded more finely, with respect to eigenvalues  of $F$. We will be mostly interested in systems in which the fermion number is bounded above and thus
\equ{
\cH=\cH^{0}\oplus \cH^{1}\oplus\cdots \oplus \cH^{n}\,,
}
where $\cH^{p}$ is spanned by all states with $F=p$ and $N$ is the maximum fermion number in the system. Then $\cH_{B}$ and $ \cH_{F}$ correspond to states with even and odd fermion number, respectively.

By definition, an operator $\cO$ has definite fermion number $f$, if
\equ{
[F,\cO]= f \cO\,.
}
We will informally say that such an operator has fermion number $F=f$. Note that the action by the operator $\cO_{h}$ on a state $\ket{s}$ with fermion number $k$ gives a state $\cO\ket{s}$ with fermion number $f+k$; $F \cO\ket{s}=(f+k)\cO\ket{s}$. An operator with $F=0$ thus preserves the fermion number of the states it acts on and the operator is block diagonal in a the basis of states organized by fermion number.



All that is required for defining supersymmetry is that $\cQ$ maps states with even fermion number to states with odd fermion number and vice versa. Thus, the supercharge $\cQ$ must have definite parity, $(-1)^{F}=-1$, but not necessarily definite fermion number $F$ (the supercharge may be given, for instance, by a sum of terms each with odd fermion number). However, in the case that $\cQ$ has  a definite fermion number and equal to $1$, i.e., 
\equ{
[F,\cQ]=\cQ\,.
}
The supercharge then acts by sending states in $\cH^{p} $ to states in $\cH^{p+1}$ and the complex \eqref{complexBF} splits into
\equ{\label{complexN}
C:\qquad 0\xrightarrow{\cQ}\cH^{0}\xrightarrow{\cQ}\cH^{1}\xrightarrow{\cQ} \cdots \xrightarrow{\cQ}\cH^{N}\xrightarrow{\cQ}0 \,,
}
where we have included the empty spaces at the ends to emphasize there are no states with $F<0$ or $F>N$. Then, one may define the cohomology groups at each level, 
\eqs{
H^{p}(\cQ)\equiv\,& \frac{\text{Ker}(\cQ): \cH^{p}\to \cH^{p+1}}{\text{Im}(\cQ): \cH^{p-1}\to \cH^{p}}\,.
}
As above, the cohomology groups are in one-to-one correspondence with the space of supersymmetric ground states with fermion number $p$, 
\equ{
 H^p(\cQ)= \cH^p_{E=0}\,.
}
The $p^{\text{th}}$ Betti number $\beta_{p}$ is defined as the dimension of the $p^{\text{th}}$ cohomology group,
\equ{
\beta_{p}\equiv \dim H^{p}(\cQ)\,.
}







\subsection{Supersymmetry in lattice systems}
\label{sec:Supersymmetry in lattice systems}

A number of interesting models of supersymmetric quantum mechanics have been studied in the literature, with applications ranging from statistical mechanics to string theory and with deep connections to algebraic topology.\footnote{For instance, a supersymmetric version of a free particle moving in a curved manifold leads to a description of de Rham cohomology and turning on a potential leads to Morse theory \cite{}. See \cite{} for a pedagogical review. \MC{complete}}  In this paper we are mostly interested in the realization of $\cN=2$ quantum mechanics in a {\it discrete} system of spins or qubits, as first discussed in \cite{Nicolai:1976xp}. It is most convenient to use the fermionic representation of states. 
% \cite{Crichigno:2020vue}, with Hilbert space
%\equ{
%\cH=(\Bbb C^{2})^{\otimes N}\,,
%}
%which is spanned by all $N$-bit strings.\footnote{More generally, one may consider a subspace $\cH\subseteq(\Bbb C^{2})^{N}$, as specified by a projector $\cP$ satisfying $[\cP,\cQ]=0$. For now we take $\cP=\Bbb I$, unless otherwise specified; see     \cite{Crichigno:2020vue} for details. } The first observation is that this space comes with a natural $\Bbb Z_{2}$-grading, 
%\equ{
%\cH=\cH^{+}\oplus\cH^{-}\,,
%}
%where $\cH^{+}$ and $\cH^{-}$ are spanned by the set of $N$-bit strings with an even and odd number of 1's, respectively. To define the action of supersymmetry in this Hilbert space, the idea is to identify these with ``bosonic'' and ``fermionic'' subspaces, i.e.,
%\eqs{\label{paritystrings}
%(-1)^{F}=\otimes_{i=1}^{N} \sigma_{z}^{i}=\begin{cases} +1 &\text{even number of 1's}\\ -1 & \text{odd number of 1's} \end{cases}
%}
%Then, we define $\cN=2$ supersymmetry in the space of qubits as  a nilpotent map $\cQ$ sending states in $\cH^{+}$ into states in $\cH^{-}$ and vice versa. 
%
%To see that this identification is consistent, and in fact rather natural, it is most convenient to work in the fermionic model of quantum computation \cite{2002AnPhy.298..210B,Ortiz:2000gc}. Recall that the Hilbert space of $N$ qubits is isomorphic to the Hilbert space of $N$ (spinless) fermions. 
In this model one considers $N$ vertices of a graph $G$, each of which can be occupied by 0 or 1 spinless fermions  (see e.g. \cite{Bravyi_2002}). A fermion at vertex $i$ is created by an operator $a_{i}^{\dagger}$ and annihilated by $a_{i}$,  satisfying the standard  anticommutation relations
\equ{
\{a_i,a_j^\dagger\}= \delta_{ij}\,,\qquad \qquad i,j\in\{1,\ldots,N\}\,,
}
$\ket{0\cdots0}$, is the state with no fermionic excitations, which is annihilated by all $a_i$, i.e.,  $a_{i}\ket{0\cdots0}=0$ for all $i$. The fermion number operator in Fock space is defined as
\equ{
F=\sum_{i=1}^{N} a^{\dagger}_{i}a_{i}\,.
}
The $2^{N}$-dimensional Fock space is then constructed by acting  with creation operators on the vacuum state, as
\equ{\label{mapstates}
\ket{n_{1}\cdots n_{N}}= (a_{1}^{\dagger})^{n_{1}}\cdots (a_{N}^{\dagger})^{n_{N}}\ket{0\cdots0}\,.
}
Note that the fundamental modes $a_i^\dagger$ are fermionic. However, the multiparticle states $\ket{n_1\cdots n_N}$ can be either bosonic or fermionic  depending on whether the total number of fermionic particles in the state is even or odd, respectively, i.e.,
\eqs{\label{paritystrings}
(-1)^{F}\ket{n_{1}\cdots n_{N}}=\begin{cases} +\ket{n_{1}\cdots n_{N}}&\text{for $\sum_{i} n_{i}\in 2\Bbb Z$}\\ -\ket{n_{1}\cdots n_{N}} &\text{for $\sum_{i} n_{i}\in 2\Bbb Z+1$} \end{cases}
}


%It is then clear from \eqref{mapstates} that fermion number in Fock space corresponds to Hamming weight in qubit space and even (odd) $N$-bit strings are indeed identified with bosonic (fermionic) states. 
%


%A systematic map between general operators in Fock space and in qubit space is obtained via a spin-$\tfrac12$ Jordan-Wigner transformation,
%\equ{\label{asigma}
%a_i \rightarrow K_{i}\,  \sigma_+^i \,, \qquad \qquad a_i^\dagger  \rightarrow \sigma_-^i K_{i}^{\dagger}  \,,
%}
%where   $\sigma_{\pm}\equiv\frac12(\sigma_{x}\pm i\sigma_{y})$ and satisfy
%\equ{\label{algsigmas}
%\sigma_{\pm}^{2}=0\,,\qquad \{\sigma_{+},\sigma_{-}\}=1\,,\qquad \{\sigma_{\pm},\sigma_{z}\}=0\,,
%}
%with $\sigma_{x,y,z}$ the standard Pauli matrices and the $K_{i}$ are non-local operators depending on $G$. In the case of a 1d graph $K_{i}=\prod_{j=1}^{i-1}(-1)^{n_{i}}$ (see, e.g., \cite{Ortiz:2000gc} and references therein for generalizations). 

Any operator in Fock space can be constructed as a polynomial in the fermionic operators $a_{i}$ and $a_{i}^{\dagger}$. The supercharge $\cQ$ must consist only of an odd number of these operators to be consistent with its fermionic nature. In the model of \cite{Nicolai:1976xp} the supercharges are cubic functions of the creation and annihilation operators. More generally one can write
\eqss{
\cQ=\sum_{i}(\alpha_{i}a_{i}^{\dagger}+\bar \alpha_{i}a_{i})+\,&\sum_{ijk}( \alpha_{ijk}a^{\dagger}_{i}a^{\dagger}_{j}a^{\dagger}_{k}+\beta_{ijk}a^{\dagger}_{i}a^{\dagger}_{j}a_{k}+\gamma_{ijk}a^{\dagger}_{i}a_{j}a_{k})  \\
+\,&\sum_{ijk}( \bar \alpha_{ijk}a_{i}a_{j}a_{k}+\bar\beta_{ijk}a_{i}a_{j}a^{\dagger}_{k}+\bar\gamma_{ijk}a_{i}a^{\dagger}_{j}a^{\dagger}_{k})+\cdots
}
%As a generalization, we consider the  ansatz,
%\equ{\label{ansatzQ}
%\cQ =  \sum_{i} a_{i}^{\dagger} \, B_{i}(a,a^{\dagger})\,, \qquad \qquad \cQ^{\dagger} =  \sum_{i}  B^{\dagger }_{i}(a,a^{\dagger})\, a_{i}\,,
%}
where  the $\alpha_{i},\bar \alpha_{i},\alpha_{ijk},\bar \alpha_{ijk}$, etc. are complex coefficients which are constrained  by the nilpotency condition \eqref{nilpQ}. Any such supercharge defines a supersymmetric Hamiltonian via \eqref{QQcom} which, by construction, is parity preserving. If each of the terms above involve at most $k$ fermionic modes we say the supercharge is $k$-local and the resulting Hamiltonian is (at most) $2k$-local. 

Note that the supercharge above has definite parity $(-1)^{F}$ but does not necessarily have a definite fermion number $F$, as it is given by the sum of terms with different odd values of $F$. We will be particularly interested in a large family of supersymmetric systems which arises from imposing two separate conditions on the supercharge.  The first is that the supercharge has definite fermion number $F=1$. We require this for later applications to the cohomology and Betti number problems. Any supercharge with $F=1$ can be written as 
\equ{
\cQ=\sum_{i}a_{i}^{\dagger}\, B_{i}(a,a^{\dagger})\,, 
}
where the $B_{i}$ are bosonic functions with $F=0$ and further constrained by the condition that the supercharge is nilpotent, $\cQ^{2}=0$. The second condition we will impose is that the supercharge is $k$-local and thus each $B^{i}$ above can be written as
\equ{
B_{i}(a,a^{\dagger})=\sum_{S_{i}} \cB_{S_{i}}(a,a^{\dagger})
}
where for each $i$,  $S_{i}\subseteq\{1,\cdots,N\}$ is a subset of $N$ vertices of size at most $k-1$, and the $\cB_{S_i}(a,a^{\dagger})$ are bosonic operators all with $F=0$ acting on the sites $S_{i}$. We thus require that each $\cB_{S_{i}}$ is a local operator in fermionic space with fermion number $F=0$. 

\paragraph{Examples.} 

The simplest model is  the 1-local supercharge
%Imposing the additional requirement that the supercharge has definite fermion number, which is usually chosen to be $F=1$, requires 
%\equ{
%\bar \alpha_{i}=\alpha_{ijk}=\gamma_{ijk}=\bar \alpha_{ijk}=\bar \beta_{ijk}=0\,,
%}
%together with the vanishing of all other terms in which the number of $a^{\dagger}$'s does not exceed those of $a$'s by one. In this case the resulting Hamiltonian is fermion number preserving. 
\equ{
\cQ=\sum_{i}a_{i}^{\dagger}\,,
}
which one can easily check squares to zero and has $F=1$. The resulting Hamiltonian, however, is proportional to the identity operator and is thus rather trivial (in particular, it has no supersymmetric ground states). Examples with a nontrivial Hamiltonian are the original models considered in \cite{Nicolai:1976xp} or the $\cN=2$ version of the SYK model \cite{Fu:2016vas}, given by
\equ{
Q=\sum_{ijk} \alpha_{ijk}a^{\dagger}_{i}a^{\dagger}_{j}a^{\dagger}_{k}\,,
}
where the $\alpha_{ijk}$ is completely antisymmetric and the supercharge has $F=3$. This model has an exponential number of supersymmetric ground states.  

Finally, a very interesting class of models is the fermion hard-core models of \cite{Fendley:2002sg}. These are specified by a choice of a graph $G=(V,E)$ and  
\equ{
\cQ=\sum_{i\in V}a_{i}^{\dagger}\, P_{i}\,,\qquad \qquad P_{i}= \prod_{j\,|\,(i,j)\in E  }(1-\hat n_{j}) \,.
}
The supercharge has $F=1$. The resulting Hamiltonian is the one in \eqref{HHC}. We will return to this model in Section~\ref{sec:Betti numbers in Topological Data Analysis} in relation to topological data analysis.

\

In the next few sections we will not focus on particular models but rather on studying the computational complexity of generic supersymmetric systems and its implications for computational topology.
%where the $B_{i}$ are a set of  operators built out of the creation/annihilation operators. Since the $a_{i}$ are fermionic, the operators $B_{i}$ must be bosonic and we thus require
%\equ{\label{bibosonic}
%[(-1)^{F},B_{i}]=0\,.
%} 
%In addition, nilpotency imposes the constraint
%\equ{\label{condq2}
%\cQ^{2}= \sum_{i,j} a_{i}^{\dagger} B_{i}(a,a^{\dagger})\, a_{j}^{\dagger} B_{j}(a,a^{\dagger})=0\,.
%}
% Different solutions to these constraints amount to different realizations of supersymmetry on a statistical mechanical system of $N$ spinless fermions. We will discuss some concrete examples below but for now we keep the discussion general and do not specify the choice of supercharges. Applying the transformation  \eqref{asigma}, we have
%\equ{\label{QQbits}
%\cQ =\sum_i  \sigma_-^i K_{i}^{\dagger}\,B_{i}\,, \qquad \qquad \cQ^\dagger =\sum_i  B_i^\dagger\, K_{i}\sigma_+^i \,,
%}
%where $B_{i}=B_{i}(K\sigma_{+},\sigma_{-}K)$. This defines the action of $\cN=2$ supersymmetry on  qubit space.
%
%Although the fermionic model provides a natural framework for justifying the identification \eqref{paritystrings} and constructing explicit representations of supersymmetry by solving \eqref{bibosonic} and \eqref{condq2}, this can also be done directly in qubit space (see \cite{Crichigno:2020vue}). Indeed, the latter will be the approach taken in Section~\ref{sec:Computational complexity} to establish the hardness of determining the lowest eigenvalue of a supersymmetric Hamiltonian. 





==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
